Isomorphism of pointed minimal systems is not classifiable by countable structures

We prove that the topological conjugacy relations both for minimal systems and pointed minimal systems are not Borel-reducible to any Borel $S_{\infty}$-action.

==> Graph_2.tex <==





\begin{figure}[h!]
\centering
\begin{tikzpicture}
\usetikzlibrary{math}

\usetikzlibrary{decorations.pathreplacing}

\node (x0) at (-3 * 0.4, 0.0)    {$\cdot$} ;
\node (x0) at (-2 * 0.4, 0.0)    {$\cdot$} ;
\node (x0) at (-1 * 0.4, 0.0)    {$\cdot$} ;
\node (00) at ( 0 * 0.4, 0.0)    {} ;
\node (01) at ( 1 * 0.4, 0.0)    {$B$} ;
\node (02) at ( 2 * 0.4, 0.0)    {} ;
\node (03) at ( 3 * 0.4, 0.0)    {} ;
\node (04) at ( 4 * 0.4, 0.0)    {$B$} ;
\node (05) at ( 5 * 0.4, 0.0)    {} ;
\node (06) at ( 6 * 0.4, 0.0)    {} ;
\node (07) at ( 7 * 0.4, 0.0)    {$A$} ;
\node (08) at ( 8 * 0.4, 0.0)    {} ;
\node (09) at ( 9 * 0.4, 0.0)    {} ;
\node (10) at (10 * 0.4, 0.0)    {$A$} ;
\node (11) at (11 * 0.4, 0.0)    {} ;
\node (12) at (12 * 0.4, 0.0)    {} ;
\node (13) at (13 * 0.4, 0.0)    {$B$} ;
\node (14) at (14 * 0.4, 0.0)    {} ;
\node (15) at (15 * 0.4, 0.0)    {} ;
\node (16) at (16 * 0.4, 0.0)    {$B$} ;
\node (17) at (17 * 0.4, 0.0)    {} ;
\node (18) at (18 * 0.4, 0.0)    {} ;
\node (19) at (19 * 0.4, 0.0)    {} ;
\node (20) at (7.2, 0.0)    {$\cdot$} ;
\node (20) at (7.6, 0.0)    {$\cdot$} ;
\node (20) at (8.0, 0.0)    {$\cdot$} ;
\node      at (3.4, -1.15) {0}       ;
\node      at (4.6, -1.15) {$p_i$}       ;
\node      at (2.2, -1.15) {$-p_i$}       ;
\draw[-] (-5 * 0.4, 0.3) -- (9, 0.3) ;
\draw[-] (-5 * 0.4, -0.3) -- (9, -0.3) ;
\draw[-] (2.2, -0.3) -- (2.2, 0.3) ;
\draw[-] (3.4, -0.3) -- (3.4, 0.3) ;
\draw[-] (5.8, -0.3) -- (5.8, 0.3) ;
\draw[-] (4.6, -0.3) -- (4.6, 0.3) ;
\draw[-] (7, -0.3) -- (7, 0.3) ;
\draw[-] (1, -0.3) -- (1, 0.3) ;
\draw[-] (-0.2, -0.3) -- (-0.2, 0.3) ;
\draw[->] (3.4, -0.3-0.5) -- (3.4, 0.3-0.75) ;
\draw[->] (4.6, -0.3-0.5) -- (4.6, 0.3-0.75) ;
\draw[->] (2.2, -0.3-0.5) -- (2.2, 0.3-0.75) ;

  
\end{tikzpicture}
\caption{corresponding pieces of $f(z)$}
\end{figure}

